Measuring the magnetic origins of solar flares, CMEs and Space Weather

We take a broad look at the problem of identifying the magnetic solar causes of space weather. With the lackluster performance of extrapolations based upon magnetic field measurements in the photosphere, we identify a region in the near UV part of the spectrum as optimal for studying the development of magnetic free energy over active regions. Using data from SORCE, Hubble Space Telescope, and SKYLAB, along with 1D computations of the near-UV (NUV) spectrum and numerical experiments based on the MURaM radiation-MHD and HanleRT radiative transfer codes, we address multiple challenges. These challenges are best met through a combination of near UV lines of bright \ion{Mg}{2}, and lines of \ion{Fe}{2} and \ion{Fe}{1} (mostly within the $4s-4p$ transition array) which form in the chromosphere up to $2\times10^4$ K. Both Hanle and Zeeman effects can in principle be used to derive vector magnetic fields. However, for any given spectral line the $\tau=1$ surfaces are generally geometrically corrugated owing to fine structure such as fibrils and spicules. By using multiple spectral lines spanning different optical depths, magnetic fields across nearly-horizontal surfaces can be inferred in regions of low plasma $\beta$, from which free energies, magnetic topology and other quantities can be derived. Based upon the recently-reported successful suborbital space measurements of magnetic fields with the CLASP2 instrument, we argue that a modest space-borne telescope will be able to make significant advances in the attempts to predict solar eruptions. Difficulties associated with blended lines are shown to be minor in an Appendix.

==> extras.tex <==

Owing to
of its enormous size
and high conductivity, free magnetic energy is able to build  quasi-statically in response to 
the sluggish motions in the photosphere
because of large (thousands of km per second) coronal Alfv\'en speeds.  With the large physical
scales of the corona, this evolution permists volume-integrated 
magnetic free energy densities to build slowly in the fashion anticipated 6 decades ago
by Gold \&{} Hoyle. 

\gdt{There were 2 other workshops in 2017. I added two papers in biblio.bib by Leka et al. in 2019 that report on the findings of one workshop, the other was part of the FLARECAST project. We may want to mention both since are more recents.}


, but
because they fail to
attempt to measure 
properties of 
magnetic fields 
directly within or at
the base of the corona



 Efforts 
are being considered for flight in space
\citep{dePontieu+others2020} with goals
which seem to overlap ours. But none has the capability to 
address the onset of magnetically-driven
eruptions by studying the magnetic field at higher atmospheric layers directly. \pgj{In the absence of rare atomic level crossings (discussed below), intensities of EUV and UV spectral lines only address what happens \textit{after} the build up of magnetic energy and stresses
has already occurred.
EUV and UV emission is
the end result of 
magnetic energy transport and dissipation, i.e. it is part of the unsolved problem of 
coronal heating. The only signature of
magnetic fields in such measurements 
results from Alfv\'en's Theorem: 
the plasma is frozen to the magnetic fields between 
dynamic reconnection events.  The brightness of the structures simply reflects the fact that heating has recently occurred somewhere within 
the defining flux surface containing the observed plasma
\citep{Bray+others1991}}. ``Loops'' and other structures therefore 
trace out just the morphology of separated flux surfaces.



The participants of the ``All-clear'' and later workshops 
\citealp{2016ApJ...829...89B,Lekaetal2019}
were well aware of both the strengths and limitations of the datasets then available.  They adopted the long time-series  data from the Michelson Doppler Imager (MDI) on the SoHO spacecraft and 
HMI instrument on
SDO 
as measures of the magnetic fields evolving above active regions.  The flaring regions were 
tracked with an ``event list'' based upon the GOES spacecraft X-ray fluxes and 
ancillary data.   The MDI instrument 
monitored line-of-sight magnetic fields 
over decades, measured in a photospheric line of \ion{Ni}{1}  6767.8 \AA.  Given the requirements summarized 
presciently so well by \cite{Gold+Hoyle1960}, and based 
on magnetic potential theory, the community attempted then to make the 
best of a set of magnetic data which by 
themselves, contain no information on the coronal magnetic field beyond 
potential fields.   They had no actual way to infer directly
magnetic \textit{free energy} above the 
photosphere  without making various other assumptions.  
The ingenious attempts to augment the data with assumptions and other
observational data are thoroughly summarized in section 4 of the paper by 
\cite{2016ApJ...829...89B}, of which 11 different methods are described that 
attempt to find correlations of MDI data properties with flare events. At least 90 publications now reference the 
article at the time of writing, 
with applications of machine and deep learning becoming popular in recent 
publications. \citep[e.g.,][]{bobracouvidat2015,Campietal2019,Jiaoetal2020,Mishizukaetal2021}  

With the launch of the SDO spacecraft 
on 10th February 2010, time series measurements of the quasi- \textit{vector} magnetic field \rce{(what does "quasi" mean here?)} over extended periods became available. With suitable ``disambiguation'' algorithms, the real vector fields could be measured at the solar photosphere. Several groups (e.g.,  \citealp{Wang+others2019}) have taken advantage of the vector capabilities of 
HMI, with some \rce{(how much?)} \gdt{(KD reported a "modest increase" with vector data, Manolis in his SDO talk showed that all the models that have the best score are based on vector not los. The best reference I found is Leka et al 2019)} improvement of the 
measures of success of flare prediction \citep{Lekaetal2019}. \gdt{Recent work has used extrapolations to find an optimal height in the region between the photosphere and the lower corona for flare prediction} \citep{Korsosetal2020}.
However, it must be recognized that

\lk{I'd delete this (non-scientific):} Given all these problems, researchers should perhaps be surprised and/or even worried if flare prediction were successful based upon such measurements.

The only way to avoid these problems is
 to measure the magnetic fields 
 well above the photosphere, either
within the corona, or at the base of the corona itself. In the latter case, 
if the magnetic energy dominates over the plasma energy, then properties of the overlying fields can be inferred 
with established techniques from measurements across
surfaces measured through spectro-polarimetry. 
Well-posed mathematical techniques 
compatible with 
the low-$\beta$ conditions where the magnetic field is
measured become valid, for example the 
force-free field 
methods and the 
magnetic virial theorem \citep{Wiegelman+Sakurai2021, Chandrasekhar1961}. \rce{This last sentence is really hard to read properly. Maybe rearrange the order of subject-verb-object so that it is more readable?}



But, all in all, it seems magnetic data 
measured only in photospheric
features are insufficient for satisfactory predictions. 


\pb{It is not clear to me what the above lists are supposed to demonstrate. I think they need to be tied to the goals of the present paper. What are the limitations of the above measurements in determining the magnetic free energy? You also mention the ``promise of DKIST'' in certain of these cases; this needs to be returned to later in the context of the proposed observations at 259-281~nm to show what the UV provides that DKIST does not.}


 to assess departures from potential fields (those 
determined by sub-surface electric current systems), and changes in topology. 

\pb{I am struggling a little bit with the logic of the end of the paragraph above and the beginning of the next. Why would one need to probe the 3D structure of the corona, but not need to do so beneath the corona? I assume this is related to the optical thinness of the corona but more explanation is needed here.}

This conclusion certainly does not exclude the other approaches, but 
it does suggest 
a primary line of attack, augmented by data from all  available strategies.


%\lk{I'm not sure if we can state that Chen et al achieve higher skill scores, at least I didn't see that from their TSS (and the other scores are affected by sample imbalance, which means not comparable because Chen et al specifically get rid of the imbalance - which by the way is not representative of the Sun). I also would recommend to cite earlier studies (that were now commented out). To be honest, I wouldn't focus so much on particular studies (apart from Bobra and Couvidat who pioneered the effort). Most of them are not comparable because of different data sets, they all optimize for one parameter (and perform equally poorly when optimizing all skill scores), and several of them claim to significantly enhance prediction, which simply is not true. }
%\tb{TEB: Again, point is not to focus on Chen et al's TSS or other scores - those really don't matter due to differences in training sets, optimization goals, etc as you point out. The point is to emphasize that their autoencoder results verify what we found with TDA: analysis of shape/topology is more skillful than magnetic field-derived quantities in predicting flares. I know this is hard for many astrophysicists to swallow, but it's verified in several studies now. \lk{can you please point me to the specific result that verifies this? I can see near equivalence (the latent space may choose the best features), but not superiority in the published results.} Start with Deshmukh et al. 2020. A more "ML-focused" paper is here: https://www.aaai.org/AAAI21Papers/IAAI-74.DeshmukhV.pdf. There has also been a recent Master's thesis (yesterday) here at CU that extends our TDA results to LSTM and ERT architectures, but that paper is still in preparation. In TDA, there is no "latent space" like in autoencoders - it's an entirely different way of quantifying feature vectors for ML input and it consistently outperforms the SHARPS parameters for flare prediction in any architecture/training/optimization scheme.}
%I.e. you can take all the DIV and CURL of the vector field you want and call those "features" but in the end, ML flare prediction is significantly more skillful when you simply focus on the evolution of the shape of the active region structures. There is also confusion in our field due to the use of the term "topology" to describe magnetic field line connectivity (e.g., Longcope, Tarr, Barnes, et al...). While field line connectivity is a kind of "topology", it is not the mathematical definition that I'm referring to here, ie. the analysis of \emph{shape} in 2-D magnetogram images. What this means for CMEx and flare prediction is that it's not all about the field measurements - you have to capture the flows and topology of the field in the chromosphere as well, i.e., imaging is as important as spectroscopy when you want to predict eruptions.}
%Similar skill scores were achieved by further studies using magnetic data \citep[e.g.,][]{floriosetal2018, liuetal2017}. 

%\citet{Berger+others2021} 
%review the current state of the art in ML solar flare prediction with particular attention paid to the problems of inherent training set imbalance and the difficulties in predicting solar flares using photospheric magnetic field data alone. They conclude that additional information gleaned from chromospheric and coronal data sources must be incorporated in any solar flare prediction system that is to break through the skill level barriers seen in current ``photosphere-only" prediction systems.  
%\lk{do we want to cite an in prep paper at such length when there are several published reviews? It sounds a little strange to me to write that a review in 2021 concludes that additional info is needed, when studies since 2018 concluded that and therefore expanded to other wavelength regions.TEB: Bit of self-advertising, I guess... But I'm not aware of any other reviews specifically focused on ML applied to solar flare prediction. If there are any then I'm happy to cite one of those instead as long as they specifically conclude that using only photospheric magnetograms for flare prediction is hopeless and frankly quite dumb - or put more nicely, there needs to be both magnetic field and flow information from higher atmospheric layers if we're ever going to get any improvement over existing methods...which is kind of the whole point of this introduction, no?. But the point is (kind of) made in the reference to Leka et al above so I'm okay with eliminating this sentence in the interest of brevity.}


%\lk{note: I believe liu et al 2019 were the first to use an LSTM for forecasting and I'd suggest to cite them too.}
%\tb{TEB: The point in bringing up Chen et al is not the LSTM (which is not a very good RNN architecture anyway due to very slow convergence...)  but to cite their autoencoder work which was novel and significant, as mentioned in the next sentence:While their skill scores are comparable to other ML-based methods, they show that CNN autoencoder ``shape-based'' features impart higher predictive skill than the magnetic field-derived quantities contained in the SHARPs metadata.}
%\lk{I agree on the autoencoder, but would rephrase to avoid lstm then, plus I'm not sure I understand your reason for inclusion because it seems to contradict their abstract: ``Effective feature extraction and feature selection with raw magnetogram data using deep learning and statistical algorithms enable us to train classification models to achieve almost as good performance as using active region parameters provided in HMI/Space-Weather HMI-Active Region Patch (SHARP) data files.''} 
%\tb{Hmm - in Chen's talk at AGU 2019 (after the paper was published) she specifically stated that the autoencoder results were superior to the SHARPS parameters, but I see now that there's no direct comparison in the paper itself. One can try to tease it out of Fig.5b vs 5a for the 12 hour forecasts, but ROC plots are not the best comparison tools...Too bad - we can't cite the paper for this finding then. Backing off to just citing it as one of the "later studies"...Also making the TDA results less bombastic - even though it's true that TDA beats SHARPS alone in all models we've tried.} \lk{thanks, the current version sounds fine to me.}
%\tb{More recently, \citep{Deshmukh+others2020} show that combining Topological Data Analysis (TDA) of the radial magnetic field structure in active regions with the SHARPs vector magnetic field metadata results in significantly higher skill scores compared to using the SHARPs metadata alone. This result implies that inclusion of high-resolution imaging of active region and flows is an important compliment to spectroscopic measurements when deducing atmospheric conditions that evolve to a flaring state. }


% I don't think this adds much to the argument (Tom Berger, TEB):
%Only modest improvements 
%in skill are associated when
%vector magnetic field data are used instead of 
%line-of-sight (LOS) fields \citep{Lekaetal2019}.  

%\tb{Are we sure we want to quote this? Basically Leka has an implicit bias to saying ``photospheric magnetic field measurements are sufficient to produce `modern' flare forecasts.'' This sentence basically asserts that "parameterizations" of the coronal field via photospheric magnetograms are ``good enough''. I disagree strongly and think that no one has yet demonstrated any flare prediction system worth 2 cents based only on photospheric magnetic field and/or continuum data. We MUST measure the chromosphere and the corona to make real progress.}
%
%\pgj{Yes Tom, the quote serves to show the [desperate] measures 
%one needs to go to to try to augment photospheric vector B fields
%with other information of dubious merit- the quote does not state 
%that these are ``good enough'' but merely states that 
%the techniques must have additional [hokey] information}
%


%\lk{I'd rephrase because they do have shown some skill score improvements, depending on the selected optimization. Suggestion: However these systems have not yet shown the required prediction accuracy that enable deployment into operational space weather forecasting systems. }\tb{TEB: "accuracy" is a technical term in this context which is the least applicable to operational efficacy - a system that always predicts "no flare" will be 99.9\% accurate but also completely useless. Nishizuka's DeFN system is in fact in operation at the NICT forecasting center so I've tried another summary sentence - let me know what you think. \lk{yes, sounds fine now, thanks.} Changed it back to cite the improvements without making any statements about operational readiness. \lk{ok}}

